Exposing Non-Atomic Methods of Concurrent Objects

Multithreaded software is typically built with specialized concurrent objects like atomic integers, queues, and maps. These objects' methods are designed to behave according to certain consistency criteria like atomicity, despite being optimized to avoid blocking and exploit parallelism, e.g., by using atomic machine instructions like compare and exchange (cmpxchg). Exposing atomicity violations is important since they generally lead to elusive bugs that are difficult to identify, reproduce, and ultimately repair. In this work we expose atomicity violations in concurrent object implementations from the most widely-used software development kit: The Java Development Kit (JDK). We witness atomicity violations via simple test harnesses containing few concurrent method invocations. While stress testing is effective at exposing violations given catalytic test harnesses and lightweight means of falsifying atomicity, divining effectual catalysts can be difficult, and atomicity checks are generally cumbersome. We overcome these problems by automating test-harness search, and establishing atomicity via membership in precomputed sets of acceptable return-value outcomes. Our approach enables testing millions of executions of each harness each second (per processor core). This scale is important since atomicity violations are observed in very few executions (tens to hundreds out of millions) of very few harnesses (one out of hundreds to thousands). Our implementation is open source and publicly available.

==> checking.tex <==
%!TEX root = draft.tex
\section{Atomicity Checking}
\label{sec:checking}

In general, checking atomicity (linearizability) for a given execution is intractable -- it has been proven to be NP-hard~\citep{DBLP:journals/siamcomp/GibbonsK97}. Being able to enumerate and check millions of executions to search for an atomicity violation is thus a big challenge. This challenge remains in place even considering ``small'' harnesses, once they contain more than 2-3 invocations. Our solution to this problem consists in checking a property weaker than linearizability for each test-harness execution but which is complete in the limit, i.e., for every violation to linearizability there exists a test-harness which exposes that violation.

We consider a fixed indexing function $invoc\text{-}index$ which for every harness $h$ fixes an order between the method invocations in $h$, i.e., for every harness $h$,
\begin{align*}
invoc\text{-}index(h): invocations(h) \rightarrow [0,\#invocations(h)-1]
\end{align*}
is a one-to-one correspondence ($invocations(h)$ is the multiset of invocations in $h$). For instance, given any harness $h=(list\text{-}invoc\text{-}seq,happens\text{-}\mathit{before})$, $invoc\text{-}index$ could order invocations as they are listed in $list\text{-}invoc\text{-}seq$. Then, we define an \emph{outcome} of a harness $h$ as a mapping $o$ from invocation indices to return values
\begin{align*}
o: [0,\#invocations(h)-1] \rightarrow \mathbb{Z}\cup\{()\}
\end{align*}
which is extracted from an execution of the harness (over the concurrent object under test) as follows: $o(i)=v\in\mathbb{Z}$ iff the invocation indexed by $i$, i.e., $invoc\text{-}index(h)^{-1}(i)$, returns $v$, and $o(i)=()$ when the invocation indexed by $i$ is of a method returning void~\footnote{We consider only executions where all the method invocations terminate.}.

%TODO DO WE NEED TO MAKE MORE PRECISE WHAT DO WE MEAN BY "CONCRETE EXECUTION OF THE HARNESS" ?

TODO EXAMPLES

Let $\mathit{outcomes}(h)$ be the set of all outcomes of $h$.  Also, let $\mathit{atomicOutcomes}(h)$ be the set of all outcomes of $h$ extracted from \emph{linearizations} of $h$, i.e., sequences of method invocations consistent with the sequences and the happens-before constraints in $h$. TODO EXAMPLE.

We say that a harness $h$ is \emph{atomic} when it generates only atomic outcomes, i.e.,
\begin{align*}
\mathit{atomic}(h)=\mathsf{true} \mbox{ iff }outcomes(h) \subseteq atomicOutcomes(h)
\end{align*}

This notion of atomicity is weaker than standard linearizability which compares \emph{histories} instead of outcomes extracted from concurrent and respectively, sequential executions. For a brief recall, 
a \emph{history} of a harness $h$ is a triple $hist=(h,o,<)$ where $o$ is an outcome extracted from an execution $e$ and $<$ is the happens-before order between invocations in $e$ (an invocation happens-before another one if it returns before the other one is called)~\footnote{Note that the happens-before order $<$ in the execution $e$ may be stronger than the one included in the harness $h$. For instance, a harness with two parallel sequences (no happens-before constraints) has executions where no two invocations overlap whose happens-before is a total order.}. Informally, a history $hist$ is \emph{linearizable} when it can be linearized to a sequence of invocations that is admitted by the object under consideration. In more precise terms, $hist=(h,o,<)$ is linearizable when there exists another history $hist'=(h,o,<')$ such that $<'$ is a total order and consistent with $<$, i.e., every two invocations ordered by $<$ are ordered in the same way by $<'$. A harness is \emph{linearizable} when all its histories are.

TODO EXAMPLE

\begin{proposition}\label{prop:lin}
A linearizable harness is atomic.
\end{proposition}
\begin{proof}
Let $o$ be an outcome of a harness $h$ extracted from an execution $e$, and $hist=(h,o,<)$ the history of $e$. By hypothesis, there exists a history $hist'=(h,o,<')$ of $h$ where $<'$ is a total order consistent with $<$. This history corresponds to an execution $e'$ which represents a linearization of $h$ and thus, $o\in atomicOutcomes(h)$.
\end{proof}

%TODO ASSUMING THAT THE OBJECT IS SEQUENTIALLY DETERMINISTIC

Note that the reverse of Proposition~\ref{prop:lin} is not true. For instance, TODO. However, the following result shows that checking atomicity of harnesses allows to discover all the linearizability violations in the limit.

\begin{theorem}
For every non-linearizable harness $h$, there exists a harness $h'$ with $\mathit{methods}(h)=\mathit{methods}(h')$ which is not atomic.
\end{theorem}
\begin{proof}
Let $h$ be a non-linearizable harness. Then, there exists a history $hist=(h,o,<)$ which is not linearizable. We define a harness $h'$ where every invocation sequence is a singleton, containing one of the invocations in $h$, and the happens-before constraints encode the order $<$ from $hist$. Assuming by contradiction that $h'$ is atomic contradicts the hypothesis that $hist$ is not linearizable.
\end{proof}

for every non-linearizable harness there exists another harness which is not at

TODO STATE COMPLETENESS

TODO SAY HOW DO WE CHECK IT CONCRETELY, WE COMPUTE A-PRIORI $sequentialOutcomesSet(h)$ AND THEN CHECK MEMBERSHIP.


%\begin{algorithm}[t]
%  \SetAlgoLined
%  \SetKwInOut{Input}{Input}
%  \Input{A test-harness $h$ and an indexing function $invoc\text{-}index$ for $h$}
%  \KwResult{$\mathsf{true}$ if $h$ has a non-atomic behaviour.}
%  $atOutSet$ $\gets$ $\mathit{atomicOutcomes}(h,invoc\text{-}index)$\;
%  \While{$out$ $\gets$ $\mathit{nextOutcome}(h,invoc\text{-}index)$}{
%       \uIf{ $out\not\in atOutSet$ }{
%            \Return $\mathsf{true}$\;
%       }
%   }    
%   \Return $\mathsf{false}$\;   
%\caption{The procedure $checkNonAtomicity$ for checking non-atomicity of a harness.}
%  \label{alg:abstractCheck}
%\end{algorithm}
%
%\begin{algorithm}[t]
%  \SetAlgoLined
%  \SetKwInOut{Input}{Input}
%  \Input{A test-harness $h$ and an indexing function $invoc\text{-}index$ for $h$}
%  \KwResult{The set of outcomes of $h$ when method invocations are atomic.}
%  $\mathit{result}$ $\gets$ $\emptyset$\;
%  \For{each linearization $lin$ of $h$}{
%     $\mathit{result}$ $\gets$ $\mathit{result}\cup\{\mathit{outcome}(h,lin)\}$\;
%   }
%   \Return $\mathit{result}$\;   
%\caption{The procedure $\mathit{atomicOutcomes}$ computing the atomic outcomes of a harness.}
%  \label{alg:abstractCheck}
%\end{algorithm}




\begin{theorem}

  TODO SAY HOW THIS CRITERION IS USEFUL

\end{theorem}


==> data/generated-tables.tex <==
---
TABLE
---
\begin{tabular}{ccllrr}
\toprule
\multicolumn{6}{c}{ConcurrentHashMap} \\
\multicolumn{2}{c}{enumeration} & \multicolumn{3}{c}{failure} & \\
\cmidrule(lr){1-2} \cmidrule(lr){3-5}
\#I, \#S, \#V & exp / gen & harness & outcome & frequency & time \\
\cmidrule(lr){1-6}
5, 2, 2 & 100 / 331,008 & \tt [put(1,1); {\bf clear}()],[put(0,1); remove(0); remove(1)] & \tt N,N,N,1 & 72 / 1,077,520 & 61s \\
4, 2, 2 & 1,700 / 24,384 & \tt [put(0,0); remove(1)],[put(1,0); {\bf contains}(0)] & \tt N,0,N,F & 6 / 1,508,770 & 593s \\
5, 2, 2 & 600 / 662,016 & \tt [get(1); {\bf containsValue}(1)],[put(1,1); put(0,1); put(1,0)] & \tt 1,F,N,N,1 & 1 / 3,993,110 & 325s \\
3, 2, 2 & 100 / 408 & \tt [put(0,1); put(1,0)],[{\bf elements}()] & \tt N,N,[0] & 3 / 1,665,650 & 33s \\
3, 2, 2 & 100 / 408 & \tt [put(0,1); put(1,0)],[{\bf entrySet}()] & \tt N,N,[1=0] & 23 / 2,688,890 & 8s \\
3, 2, 2 & 100 / 408 & \tt [containsKey(1); {\bf isEmpty}()],[put(1,0)] & \tt T,T,N & 134 / 6,970,780 & 8s \\
3, 2, 2 & 100 / 408 & \tt [put(0,1); put(1,1)],[{\bf keySet}()] & \tt N,N,[1] & 18 / 5,048,060 & 17s \\
3, 2, 2 & 100 / 408 & \tt [{\bf keys}()],[put(0,1); put(1,1)] & \tt [1],N,N & 13 / 1,721,300 & 16s \\
3, 2, 2 & 100 / 408 & \tt [containsKey(1); {\bf mappingCount}()],[put(1,0)] & \tt T,0,N & 125 / 5,511,280 & 8s \\
3, 2, 2 & 100 / 3,264 & \tt [{\bf putAll}(\{0=0,1=0\})],[remove(0); get(1)] & \tt 0,N & 2 / 2,099,190 & 12s \\
3, 2, 2 & 100 / 408 & \tt [get(1); {\bf size}()],[put(1,1)] & \tt 1,0,N & 4 / 6,533,430 & 8s \\
3, 2, 2 & 100 / 408 & \tt [put(0,1); put(1,1)],[{\bf toString}()] & \tt N,N,{1=1} & 120 / 3,948,560 & 27s \\
3, 2, 2 & 100 / 408 & \tt [put(0,1); put(1,0)],[{\bf values}()] & \tt N,N,[0] & 99 / 2,836,280 & 25s \\
\midrule
\multicolumn{6}{c}{ConcurrentSkipListMap} \\
\cmidrule(lr){1-6}
4, 2, 2 & 300 / 12,192 & \tt [{\bf clear}(); put(1,0); put(1,0)],[put(0,0)] & \tt N,N,N & 1,000 / 5,067,830 & 102s \\
4, 2, 2 & 1,700 / 24,384 & \tt [put(0,0); remove(1)],[put(1,0); {\bf containsValue}(0)] & \tt N,0,N,F & 2 / 3,418,150 & 585s \\
4, 2, 2 & 200 / 12,192 & \tt [put(0,1); {\bf entrySet}()],[put(0,0); put(1,1)] & \tt N,[0=1,1=1],1,N & 148 / 1,271,070 & 52s \\
3, 2, 2 & 100 / 3,264 & \tt [put(0,0); containsKey(1)],[{\bf putAll}(\{0=1,1=1\})] & \tt 1,F & 25 / 1,847,900 & 10s \\
4, 2, 2 & 1,200 / 12,192 & \tt [put(0,1); remove(1)],[put(1,1); {\bf size}()] & \tt N,1,N,0 & 1 / 3,898,810 & 408s \\
5, 2, 2 & 600 / 662,016 & \tt [put(0,1); containsKey(0); put(0,0); put(1,0)],[{\bf tailMap}(0)] & \tt N,T,1,N,{0=1,1=0} & 56 / 2,291,450 & 341s \\
4, 2, 2 & 200 / 12,192 & \tt [put(0,1); put(1,1)],[put(0,0); {\bf toString}()] & \tt 0,N,N,{0=0,1=1} & 8 / 2,269,590 & 48s \\
4, 2, 2 & 200 / 12,192 & \tt [put(0,1); put(1,1)],[put(0,0); {\bf values}()] & \tt 0,N,N,[0,1] & 12 / 2,069,060 & 71s \\
\midrule
\multicolumn{6}{c}{ConcurrentSkipListSet} \\
\cmidrule(lr){1-6}
3, 2, 2 & 100 / 640 & \tt [{\bf addAll}([0,1])],[contains(0); add(1)] & \tt T,T,T & 2,645 / 3,589,490 & 9s \\
4, 2, 2 & 500 / 2,816 & \tt [add(0)],[add(1); {\bf clear}(); add(1)] & \tt T,T,F & 9 / 2,942,870 & 155s \\
4, 2, 2 & 500 / 11,264 & \tt [add(1); {\bf containsAll}([1,0])],[remove(1); add(0)] & \tt T,T,T,T & 360 / 3,055,220 & 164s \\
5, 2, 3 & 9,100 / 155,520 & \tt [remove(0); remove(1)],[add(0); add(1); {\bf headSet}(2)] & \tt T,T,T,T,[0] & 106 / 1,643,840 & 3282s \\
4, 2, 2 & 400 / 2,816 & \tt [add(0); contains(1)],[add(1); poll()] & \tt T,T,T,1 & 2 / 1,621,280 & 122s \\
4, 2, 2 & 200 / 2,816 & \tt [add(1); contains(0)],[add(0); {\bf pollLast}()] & \tt T,T,T,0 & 4 / 2,262,770 & 64s \\
4, 2, 2 & 100 / 11,264 & \tt [{\bf removeAll}([0,0])],[add(0); add(0); contains(0)] & \tt T,T,T,F & 86 / 3,625,490 & 28s \\
3, 2, 2 & 100 / 640 & \tt [remove(0)],[add(0); {\bf retainAll}([1,1])] & \tt T,T,T & 2,659 / 3,380,760 & 12s \\
4, 2, 2 & 2,500 / 2,816 & \tt [add(0); remove(1)],[add(1); {\bf size}()] & \tt T,T,T,0 & 1 / 2,785,410 & 878s \\
4, 2, 4 & 7,600 / 131,072 & \tt [{\bf subSet}(0,3)],[add(1); add(0); add(2)] & \tt [1,2],T,T,T & 836 / 1,970,550 & 2780s \\
5, 2, 2 & 1,000 / 90,368 & \tt [{\bf tailSet}(0)],[add(1); add(0); remove(0); remove(1)] & \tt [0],T,T,T,T & 631 / 2,340,020 & 350s \\
5, 2, 2 & 1,100 / 45,184 & \tt [remove(0); remove(1)],[add(0); add(1); {\bf toArray}()] & \tt T,T,T,T,[0] & 1 / 739,050 & 388s \\
5, 2, 2 & 100 / 45,184 & \tt [add(0); add(1); {\bf toString}()],[remove(0); remove(1)] & \tt T,T,[0],T,T & 23 / 1,843,310 & 36s \\
\midrule
\multicolumn{6}{c}{ConcurrentLinkedQueue} \\
\cmidrule(lr){1-6}
4, 2, 2 & 300 / 894 & \tt [poll()],[offer(1); offer(0); {\bf clear}()] & \tt 0,T,T & 1,289 / 4,209,580 & 84s \\
4, 2, 2 & 500 / 3,576 & \tt [poll(); offer(1)],[offer(0); {\bf containsAll}([0,1])] & \tt 0,T,T,T & 9 / 4,120,090 & 170s \\
3, 2, 2 & 100 / 312 & \tt [offer(1); poll()],[{\bf removeAll}([1,1])] & \tt T,1,T & 964 / 4,665,060 & 10s \\
3, 2, 2 & 100 / 312 & \tt [poll()],[offer(1); {\bf retainAll}([0,0])] & \tt 1,T,T & 8,222 / 5,328,260 & 10s \\
4, 2, 2 & 100 / 894 & \tt [poll(); offer(0)],[offer(1); {\bf size}()] & \tt 1,T,T,2 & 3 / 3,458,050 & 13s \\
4, 2, 2 & 100 / 894 & \tt [{\bf toArray}()],[offer(1); poll(); offer(0)] & \tt [1,0],T,1,T & 23 / 1,340,340 & 8s \\
4, 2, 2 & 100 / 894 & \tt [offer(0); poll(); offer(0)],[{\bf toString}()] & \tt T,0,T,[0,0] & 21 / 3,845,190 & 18s \\
\midrule
\multicolumn{6}{c}{LinkedTransferQueue} \\
\cmidrule(lr){1-6}
3, 2, 2 & 100 / 312 & \tt [poll(); poll()],[{\bf addAll}([1,0])] & \tt 1,N,T & 40 / 4,365,650 & 15s \\
4, 2, 2 & 300 / 894 & \tt [poll()],[offer(1); offer(0); {\bf clear}()] & \tt 0,T,T & 1,058 / 4,283,910 & 105s \\
4, 2, 2 & 500 / 3,576 & \tt [poll(); offer(1)],[offer(0); {\bf containsAll}([0,1])] & \tt 0,T,T,T & 10 / 4,384,580 & 166s \\
3, 2, 2 & 100 / 312 & \tt [offer(0); poll()],[{\bf removeAll}([0,0])] & \tt T,0,T & 21,385 / 4,968,110 & 9s \\
5, 2, 2 & 100 / 37,560 & \tt [poll(); peek(); offer(1)],[offer(0); {\bf retainAll}([1,1])] & \tt 0,N,T,T,T & 38,473 / 3,610,180 & 14s \\
4, 2, 2 & 100 / 894 & \tt [{\bf size}()],[offer(0); poll(); offer(1)] & \tt 2,T,0,T & 13 / 3,475,350 & 21s \\
4, 2, 2 & 100 / 894 & \tt [{\bf toArray}()],[offer(1); poll(); offer(0)] & \tt [1,0],T,1,T & 103 / 322,400 & 22s \\
4, 2, 2 & 100 / 894 & \tt [poll(); offer(1)],[offer(1); {\bf toString}()] & \tt 1,T,T,[1,1] & 55 / 1,867,010 & 17s \\
\bottomrule
\end{tabular}
---
TABLE
---
\begin{tabular}{ccllrr}
\toprule
\multicolumn{6}{c}{LinkedBlockingQueue} \\
\multicolumn{2}{c}{enumeration} & \multicolumn{3}{c}{failure} & \\
\cmidrule(lr){1-2} \cmidrule(lr){3-5}
\#I, \#S, \#V & exp / gen & harness & outcome & frequency & time \\
\cmidrule(lr){1-6}
3, 2, 2 & 100 / 312 & \tt [{\bf addAll}([1,1])],[poll(); peek()] & \tt T,1,N & 537 / 2,683,060 & 9s \\
5, 2, 2 & 1,600 / 9,390 & \tt [offer(1); {\bf clear}(); offer(0)],[peek(); poll()] & \tt T,T,0,N & 1 / 2,153,170 & 557s \\
4, 2, 2 & 100 / 3,576 & \tt [offer(1); {\bf containsAll}([1,0])],[poll(); offer(0)] & \tt T,T,1,T & 107 / 2,428,020 & 22s \\
6, 2, 2 & 1,100 / 186,108 & \tt [offer(0); peek(); peek()],[poll(); offer(1); {\bf contains}(0)] & \tt T,1,N,0,T,F & 1 / 1,756,190 & 406s \\
5, 2, 2 & 1,700 / 9,390 & \tt [poll(); offer(0)],[offer(1); peek(); {\bf isEmpty}()] & \tt 1,T,T,0,T & 1 / 3,137,600 & 604s \\
5, 2, 2 & 1,500 / 9,390 & \tt [poll(); offer(0)],[offer(1); peek(); {\bf remainingCapacity}()] & \tt 1,T,T,0,2147483647 & 1 / 2,259,160 & 532s \\
3, 2, 2 & 100 / 312 & \tt [{\bf removeAll}([0,1])],[offer(0); poll()] & \tt T,T,0 & 245,899 / 2,416,360 & 9s \\
5, 2, 2 & 5,300 / 18,780 & \tt [offer(1); peek(); peek()],[{\bf remove}(1); offer(0)] & \tt T,0,N,T,T & 1 / 2,097,120 & 1917s \\
3, 2, 2 & 100 / 312 & \tt [{\bf retainAll}([0,0])],[offer(1); poll()] & \tt T,T,1 & 181,760 / 2,212,120 & 8s \\
5, 2, 2 & 1,500 / 9,390 & \tt [poll(); offer(0)],[offer(1); peek(); {\bf size}()] & \tt 1,T,T,0,0 & 1 / 2,139,590 & 536s \\
6, 2, 2 & 32,400 / 93,054 & \tt [{\bf toArray}(); poll(); offer(1)],[offer(0); peek(); poll()] & \tt [],0,T,T,1,N & 1 / 565,500 & 12179s \\
6, 2, 2 & 3,500 / 93,054 & \tt [poll(); offer(1)],[offer(0); peek(); peek(); {\bf toString}()] & \tt 0,T,T,1,N,[1] & 1 / 1,459,580 & 1267s \\
\midrule
\multicolumn{6}{c}{ArrayBlockingQueue} \\
\cmidrule(lr){1-6}
3, 2, 2 & 100 / 312 & \tt [{\bf addAll}([0,0])],[poll(); poll()] & \tt T,0,N & 251 / 3,434,740 & 10s \\
4, 2, 2 & 500 / 3,576 & \tt [poll(); offer(1)],[offer(0); {\bf containsAll}([0,1])] & \tt 0,T,T,T & 5,860 / 2,042,060 & 156s \\
3, 2, 2 & 100 / 312 & \tt [offer(0); poll()],[{\bf removeAll}([1,0])] & \tt T,0,T & 26,798 / 1,279,280 & 8s \\
3, 2, 2 & 100 / 312 & \tt [poll()],[offer(1); {\bf retainAll}([0,0])] & \tt 1,T,T & 1,119 / 2,087,100 & 9s \\
\midrule
\multicolumn{6}{c}{PriorityBlockingQueue} \\
\cmidrule(lr){1-6}
3, 2, 2 & 100 / 312 & \tt [peek(); {\bf addAll}([1,0])],[poll()] & \tt N,T,1 & 10,288 / 3,062,920 & 9s \\
4, 2, 2 & 100 / 3,576 & \tt [offer(1); {\bf containsAll}([1,0])],[poll(); offer(0)] & \tt T,T,1,T & 8,655 / 2,916,430 & 26s \\
3, 2, 2 & 100 / 312 & \tt [poll()],[offer(0); {\bf removeAll}([0,0])] & \tt 0,T,T & 5,522 / 2,625,610 & 11s \\
3, 2, 2 & 100 / 312 & \tt [{\bf retainAll}([1,1])],[offer(0); poll()] & \tt T,T,0 & 7,990 / 2,968,360 & 20s \\
\midrule
\multicolumn{6}{c}{LinkedBlockingDeque} \\
\cmidrule(lr){1-6}
3, 2, 2 & 100 / 384 & \tt [{\bf addAll}([1,0])],[poll(); peek()] & \tt T,1,N & 9,832 / 2,981,050 & 9s \\
4, 2, 2 & 600 / 4,096 & \tt [offer(1); {\bf containsAll}([1,0])],[poll(); offer(0)] & \tt T,T,1,T & 4,177 / 2,555,780 & 206s \\
3, 2, 2 & 100 / 384 & \tt [offer(1); {\bf removeAll}([1,0])],[poll()] & \tt T,T,1 & 11,613 / 3,146,040 & 8s \\
3, 2, 2 & 100 / 384 & \tt [{\bf retainAll}([0,0])],[offer(1); poll()] & \tt T,T,1 & 84,882 / 3,893,750 & 18s \\
\midrule
\multicolumn{6}{c}{ConcurrentLinkedDeque} \\
\cmidrule(lr){1-6}
3, 2, 2 & 200 / 156 & \tt [poll()],[{\bf addFirst}(0); offer(1)] & \tt 1,T & 163 / 5,461,590 & 42s \\
4, 2, 2 & 200 / 894 & \tt [poll()],[offer(1); offer(0); {\bf clear}()] & \tt 0,T,T & 985 / 4,391,760 & 55s \\
4, 2, 2 & 100 / 3,576 & \tt [poll(); offer(1)],[offer(0); {\bf containsAll}([0,1])] & \tt 0,T,T,T & 7 / 3,882,720 & 28s \\
4, 2, 2 & 100 / 894 & \tt [offer(1); {\bf getLast}()],[offer(0); poll()] & \tt T,E,T,1 & 18 / 4,236,420 & 28s \\
3, 2, 2 & 200 / 156 & \tt [{\bf offerFirst}(0); offer(1)],[poll()] & \tt T,T,1 & 23 / 4,906,360 & 44s \\
4, 2, 2 & 100 / 894 & \tt [offer(1); {\bf peekLast}()],[offer(0); poll()] & \tt T,N,T,1 & 22 / 3,540,930 & 17s \\
4, 2, 2 & 100 / 894 & \tt [offer(0); {\bf pollLast}()],[offer(0); poll()] & \tt T,N,T,0 & 50 / 3,645,870 & 12s \\
3, 2, 2 & 100 / 312 & \tt [offer(0); poll()],[{\bf removeAll}([1,0])] & \tt T,0,T & 7,792 / 4,918,210 & 9s \\
4, 2, 2 & 300 / 1,788 & \tt [offer(0); {\bf removeLastOccurrence}(0)],[offer(0); poll()] & \tt T,F,T,0 & 90 / 3,975,720 & 95s \\
4, 2, 2 & 100 / 894 & \tt [offer(0); {\bf removeLast}()],[offer(0); poll()] & \tt T,E,T,0 & 18 / 3,435,730 & 23s \\
3, 2, 2 & 100 / 312 & \tt [offer(0); {\bf retainAll}([1,1])],[poll()] & \tt T,T,0 & 6,620 / 4,982,960 & 10s \\
4, 2, 2 & 100 / 894 & \tt [offer(1); poll(); offer(1)],[{\bf size}()] & \tt T,1,T,2 & 1 / 3,817,410 & 26s \\
4, 2, 2 & 100 / 894 & \tt [offer(1); poll(); offer(1)],[{\bf toArray}()] & \tt T,1,T,[1,1] & 68 / 2,156,940 & 9s \\
4, 2, 2 & 100 / 894 & \tt [poll(); offer(1)],[offer(0); {\bf toString}()] & \tt 0,T,T,[0,1] & 236 / 2,790,900 & 22s \\
\bottomrule
\end{tabular}
---
frequencies
{
  "count": 87,
  "avg": 0.003151185114787782,
  "min": 2.504313680314341e-7,
  "med": 0.00019732311462697052,
  "max": 0.10176422387392607
}
frequencies (without *All)
{
  "count": 55,
  "avg": 0.000048892491783525936,
  "min": 2.504313680314341e-7,
  "med": 0.000030390826022651296,
  "max": 0.0004242470376290883
}
frequencies (without *All, clear, hashCode)
{
  "count": 48,
  "avg": 0.00003424917787075758,
  "min": 2.504313680314341e-7,
  "med": 0.000029458867386891338,
  "max": 0.0004242470376290883
}


==> search.tex <==
%!TEX root = draft.tex
\section{Test-Harness Search}
\label{sec:search}

Our basic approach to checking non-atomicity of a method, as outlined by the abstract algorithm in Algorithm~\ref{alg:abstract}, is to search for a test-harness invoking the core methods plus the method under test that exposes an atomicity violation. We focus in this section on the test-harness search delegating the description of atomicity checking (the predicate $\mathit{atomic}$) to Section~\ref{sec:checking}. 

In general, atomicity violations are quite rare, they may occur once in hundreds of thousands or millions of executions (see Section~\ref{sec:experiments} for more details). Finding a harness which has a big enough rate of violations to be approached using testing is an important challenge and needs automation. For instance, TODO GIVE ALTERNATIVES TO CONTAINS-VALUE HARNESS

We automate the test-harness search using a prioritization scheme that enumerates harnesses in an increasing order with respect to the number of method invocations, the number of values used as parameters in those invocations, and the number of different threads used to make those invocations. Just to simplify the formalization, we assume that methods' parameters and return values are objects that can be instantiated with integers. 

We define harnesses as partially-ordered sets of sequences of method invocations represented concretely as words accepted by the following grammar:
\begin{align*}
%input & ::=  k \ |\ input,input \mbox{ where $k\in\mathbb{Z}$}\\
invoc & ::=  m(argument^*) \mbox{ where $m$ is a method name and $argument\in \mathbb{Z}$} \\
invoc\text{-}seq & ::=  invoc \ |\ invoc\text{-}seq; invoc\text{-}seq \\
list\text{-}invoc\text{-}seq & ::= [invoc\text{-}seq]\ | \ list\text{-}invoc\text{-}seq, list\text{-}invoc\text{-}seq \\ % \ |\ list\text{-}invoc\text{-}seq, list\text{-}invoc\text{-}seq \\
happens\text{-}\mathit{before} & ::= i < j \ |\ happens\text{-}\mathit{before}, happens\text{-}\mathit{before} \mbox{ where $i,j\in\mathbb{N}$}\\
harness & ::= list\text{-}invoc\text{-}seq,\{happens\text{-}\mathit{before}\}
\end{align*}
This grammar generates pairs formed of a list of invocation sequences $list\text{-}invoc\text{-}seq$ together with happens-before constraints between those sequences. The happens-before constraints are a list of constraints $i<j$ interpreted as the $i$th sequence in $list\text{-}invoc\text{-}seq$ happens-before the $j$th sequence. The following are examples of harnesses generated by this grammar:
\begin{align}
&{\tt[put(0,0)]},\ \ {\tt [clear(); put(1,1); containsKey(1)]} \label{eq:harn1} \\ 
&{\tt[put(0,0); put(2,0)]},\ \ {\tt [clear(); put(1,1)]} \label{eq:harn2} \\ 
&{\tt[put(0,0); put(2,0)]},\ \ {\tt [clear(); put(1,1); containsKey(1); get(2)]} \label{eq:harn3} \\ 
&{\tt[put(0,0); put(2,0)]},\ \ {\tt [clear(); put(1,1); containsKey(1); get(2)]}, \ \ {\tt [put(3,1)]},\ \ \{0 < 2, 1 < 2\} \label{eq:harn4}
\end{align}


A harness corresponds to a program where every sequence of invocations is executed in a different thread. Figure~\ref{fig:harness} gives a concrete implementation of the harness in (\ref{eq:harn1}) where the methods {\tt Sequence1} and {\tt Sequence2} will be executed in two different threads. Happens-before constraints $i<j$ are implemented using for instance condition variables: the sequence $j$ awaits a signal placed at the end of the sequence $i$.

We assume that harnesses are words accepted by this grammar that satisfy obvious well-formedness conditions, i.e., the list of arguments in every invocation is consistent with the method signature, and the list of happens-before constraints uses values $i$ and $j$ which are smaller than the length of $list\text{-}invoc\text{-}seq$ and defines a strict partial-order.

%For a sequence $\sigma$, let $\mathsf{len}(\sigma)$ denote its length.  harness $h=[list\text{-}invoc\text{-}seq,hb]$, let 
%\begin{align*}
%\#\mathit{sequences}(h)=\mathsf{len}(list\text{-}invoc\text{-}seq)\quad\quad  &
%\#\mathit{invocations}(h)=\sum_{i=0}^{\mathsf{len}(list\text{-}invoc\text{-}seq)} \mathsf{len}(list\text{-}invoc\text{-}seq[i])\\
%& \#\mathit{values}(h)=|\bigcup_{i=0}^{\mathsf{len}(list\text{-}invoc\text{-}seq)} \bigcup_{j=0}^{\mathsf{len}(list\text{-}invoc\text{-}seq[i])} \mathsf{inputSet}(list\text{-}invoc\text{-}seq[i][j]) |
%\end{align*}


For a harness $h=(list\text{-}invoc\text{-}seq,happens\text{-}\mathit{before})$, let $\mathit{methods}(h)$ be the set of method names used in $list\text{-}invoc\text{-}seq$, $\mathit{values}(h)$ the set of different arguments to the invocations in $list\text{-}invoc\text{-}seq$, $\#\mathit{sequences}(h)$ the length of $list\text{-}invoc\text{-}seq$, and $\#\mathit{invocations}(h)$ the total number of invocations in $list\text{-}invoc\text{-}seq$. For instance, for the harness $h$ in (\ref{eq:harn4}), we have $\mathit{methods}(h)=\{{\tt put}, {\tt clear}, {\tt containsKey}, {\tt get}\}$, $\mathit{values}(h)=\{ {\tt 0}, {\tt 1}, {\tt 2}, {\tt 3}\}$, $\#\mathit{sequences}(h)=3$, and $\#\mathit{invocations}(h)=7$.

\begin{algorithm}[t]
  \SetAlgoLined
  \SetKwInOut{Input}{Input}
  \Input{A concurrent object with atomic core $\mathit{Core}$, and a method $m$ of this object}
  \KwResult{$\mathsf{NON\text{-}ATOMIC}$ iff $m$ is non-atomic.}
  $(invoc,val,seq)$ $\gets$ $(0,0,0)$ \;
  \While{true}{
       $H$ $\gets$ $constructHarnesses ( \mathit{Core}\cup\{m\}, invoc,val,seq )$\;
       $\mathit{shuffle}(H)$\;
       \For{each harness $h\in H$}{
           \uIf{not $\mathit{atomic}( h )$}{
              \Return $\mathsf{NON\text{-}ATOMIC}$\;
           }
	}
	$(invoc,val,seq)$ $\gets$ $\mathit{nextParams()}$ \;
  }
\caption{Abstract algorithm for checking non-atomicity of a method.}
  \label{alg:abstract}
\end{algorithm}

Algorithm~\ref{alg:abstract} enumerates increasing assignments for the non-fixed parameters of $constructHarnesses$ which are generated by the function $\mathit{nextParams()}$. The latter can be any function returning triples of natural numbers satisfying the property that for any tuple $(i,v,s)\in \mathbb{N}^3$ it eventually returns a triple $(i',v',s')$ which is greater than $(i,v,s)$ component-wise. An instance of $\mathit{nextParams()}$ incrementing atomically each parameter, i.e., returning a sequence of triples $(1,1,1)$, $(2,2,2)$, $(3,3,3)$, $\ldots$ would satisfy this assumption. For some fixed set of parameters, the function $constructHarnesses$ returns the following set of harnesses:
\begin{align*}
constructHarnesses ( \mathit{Core}\cup\{m\}, invoc,val,seq)= \{ h\mbox{ a well-formed harness}\ \mid\ & \mathit{methods}(h)=\mathit{Core}\cup\{m\}, \\
& \#\mathit{invocations}(h)=invoc, \\
& \mathit{values}(h)=[0,val-1], \\
& \#\mathit{sequences}(h)=seq\}
\end{align*}
We implicitly assume that the concurrent objects under test are data-independent in the sense that any behavior with some number of distinct values $val$ can be captured when the values are taken from the interval $[0,val-1]$. The set of harnesses returned by $constructHarnesses$ is clearly finite for any given parameter assignment.

For instance, when checking the atomicity of the method {\tt clear} of {\tt ConcurrentSkipListMap}, the output of the function $constructHarnesses( \{{\tt put}, {\tt remove}, {\tt get}, {\tt containsKey}, {\tt clear}\},4,2,2)$ contains the harnesses listed in Figure~\ref{}TODO.
%\begin{align*}
%[{\tt put}(0,0); {\tt remove}(1),\ \ {\tt put}(1,0); {\tt containsValue}(0)]
%\end{align*}
%TODO ADD SOME MORE FROM THE EXAMPLES IN THE BEGINNING OF THE SECTION (SAY THAT THERE ARE NO HAPPENS-BEFORE CONSTRAINTS)

The definition of $constructHarnesses$ given above supports many optimizations that we implement in our tool. As it is, it returns many redundant harnesses which may have a negative impact on the time to find an atomicity violation. A first obvious optimization is to perform some symmetry reduction. We say that two harness are \emph{symmetric} iff one is obtained from the other by changing the order between invocation sequences and accordingly, applying a renaming on the happens-before constraints. For instance, the following is symmetric to the harness in (\ref{eq:harn4}):
\begin{align*}
%[{\tt put}(0,0); {\tt remove}(1),\ \ {\tt put}(1,0); {\tt containsValue}(0)] \\
%[{\tt put}(1,0); {\tt containsValue}(0),\ \ {\tt put}(0,0); {\tt remove}(1)]
&{\tt [put(3,1)]}, \ \ {\tt[put(0,0); put(2,0)]},\ \ {\tt [clear(); put(1,1); containsKey(1); get(2)]},\ \ \{1 < 0, 2 < 0\} \label{eq:harn4}
\end{align*}
Then, the output of the function $constructHarnesses$ is constrained such that it doesn't contain symmetric harnesses. 

Besides this optimization which is agnostic to our verification problem, we consider more specific optimizations like excluding harnesses that contain only read-only invocations, for instance, excluding the harness ${\tt [get(0); containsKey(1)]},\ {\tt [get(1); isEmpty()]}$,
%\begin{align*}
%{\tt [get(0); containsKey(1)]},\ \ {\tt [get(1); isEmpty()]} 
%\end{align*}
and excluding harnesses where the method under test for atomicity is read-only, e.g., {\tt isEmpty}, and forbidden from executing in parallel with update methods from the atomic core, e.g., 
\begin{align*}
{\tt [get(0); remove(1)]},\ \ {\tt [put(0,1); put(1,1)]},\ \ {\tt [get(1); isEmpty()]},\ \ \{0 < 2, 1 < 2\}.
\end{align*}
The last two optimizations rely on a user provided classification of the object's methods into read-only and updates depending on whether they modify or not the object's internal state. For instance, in the case of {\tt ConcurrentSkipListMap} we have used the following classification:
\begin{align*}
\text{read-only}\,: &\  {\tt get}, {\tt containsKey}, {\tt ceilingKey}, {\tt floorKey}, {\tt firstKey}, {\tt lastKey}, {\tt higherKey}, {\tt lowerKey}, {\tt keySet}, \\
& {\tt isEmpty}, {\tt containsValue}, {\tt entrySet}, {\tt values}, {\tt tailMap}, {\tt headMap}, {\tt subMap}, {\tt size}, {\tt toString}\\
\text{updates}\,: &\ {\tt put}, {\tt remove}, {\tt putIfAbsent}, {\tt replace}, {\tt putAll}, {\tt clear} 
\end{align*}
The harness search is made probabilistic using the function $\mathit{shuffle}$ that performs a randomized shuffling of the set of harnesses returned by $constructHarnesses$. 

Since the function $\mathit{nextParams()}$ doesn't enumerate all the possible parameter assignments it may miss some harnesses. For instance, the fist output of this function may be $(2,4,3)$

\begin{theorem}

  TODO MAYBE CHARACTERIZE COMPLETENESS OF SEARCH?

\end{theorem}

